Maximum Entropy Property of Discrete-time Stable Spline Kernel

In this paper, the maximum entropy property of the discrete-time first-order stable spline kernel is studied. The advantages of studying this property in discrete-time domain instead of continuous-time domain are outlined. One of such advantages is that the differential entropy rate is well-defined for discrete-time stochastic processes. By formulating the maximum entropy problem for discrete-time stochastic processes we provide a simple and self-contained proof to show what maximum entropy property the discrete-time first-order stable spline kernel has.

==> header.tex <==
% header file

\usepackage{amsmath,graphicx}
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
\usepackage{tikz}
\usepackage{url}
\newcommand{\displaycomments}

\ifdefined\displaycomments
\newcommand{\note}[1]{\textcolor{red}{\emph{#1}}}
\else
\newcommand{\note}[1]{}
\fi

%\usepackage{url}
%\usepackage[T1]{fontenc}
%\usepackage[isolatin]{inputenc}
\usepackage{xspace}
%\usepackage[squaren]{SIunits}
\usepackage{amsmath}
\usepackage{amsthm}
%\usepackage{amsthm}
\usepackage{amssymb}
%\usepackage{natbib}
\usepackage{graphicx}      % include this line if your document contains figures
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{cite}
\usetikzlibrary{arrows}
%\usepackage{pgfplots}
%\numberwithin{equation}{section}
%\usepackage{SIunits}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\newtheorem{cor}{Corollary}
\newtheorem{mydef}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{theo}{Theorem}
\newtheorem{prop}{Proposition}

%\renewcommand{\d}{\operatorname{d}}
\renewcommand{\d}{\:{\rm{d}}} 
\newcommand{\E}{\mathop{\mathbb E}}
\newcommand{\Tr}{\operatorname{Tr}}
\newcommand{\NormalGamma}{\operatorname{NormalGamma}}
\newcommand{\GaussianGamma}{\operatorname{GaussianGamma}}
\newcommand{\GIW}{\operatorname{GIW}}
\newcommand{\B}{\operatorname{B}}
\newcommand{\Bern}{\operatorname{Bern}}
\newcommand{\Exp}{\operatorname{Exp}}
\newcommand{\Weibull}{\operatorname{Weibull}}
\newcommand{\Rayleigh}{\operatorname{Rayleigh}}
\newcommand{\Laplace}{\operatorname{Laplace}}
\newcommand{\Gam}{\operatorname{Gamma}}
\newcommand{\Dir}{\operatorname{Dir}}
\newcommand{\IGam}{\operatorname{IGamma}}
\newcommand{\ISE}{\operatorname{ISE}}
\DeclareMathOperator*{\round}{round}
\renewcommand{\t}[1]{\mathrm{T}#1}
\newcommand{\N}{\mathcal{N}}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\aka}{a.k.a.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\cf}{c.f.,\xspace}
\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\diag}{\operatorname{Diag}}
\renewcommand{\baselinestretch}{0.9}
\usepackage{cite} % Loading the cite package will result in citation numbers being automatically sorted and properly "ranged". i.e., [1], [9], [2], [7], [5], [6] (without using cite.sty) will become: [1], [2], [5]--[7], [9] (using cite.sty)
\usepackage{stfloats}
\usepackage{amsmath}

\def\x{{\mathbf x}}
\def\L{{\cal L}}

%\usepackage{setspace}
%%\setstretch{0.941291}
%\setstretch{0.89}
\newcommand{\tablecaption}[1] {\caption{#1: Pairwise comparison of three reduction algorithms with respect to the KLD and ISE between the original mixture and the approximate mixture reduced incrementally. The number of remaining components in the approximate mixture is shown by \textbf{M} in the left column. The quantity in each element is the decimal logarithm of the $p-$value of the two sided Wilcoxon rank sum test. When the difference between the two reduction algorithms is statistically significant ($p$-value $<1\%$) the symbol corresponding to the  algorithm with smaller median error is given next to the $p$-value.}}

\newcommand{\figurecaption}[1] {\caption{Mixture of #1: A realization of the original mixture density and its approximations are illustrated. The original mixture density (black solid line) and its components (black dashed line) are given. In the sub-figures AKL, SKL and ISE are used to approximate the original mixture which has 25 component densities with mixtures with 3 component densities. The approximate densities (thick dashed lines)  and their components (thin dashed line) are drawn in different colors; red(AKL), green(SKL) and blue(ISE). AKL is used in the left sub-figure, SKL is used in the center sub-figure  and ISE is used in the right sub-figure. The reduced mixture in the right sub-figure is not rescaled after possible pruning steps and is plotted as it is used in the ISE algorithm. }}

\newcommand{\figurecaptiontime}[1] {\caption{#1: The average cycle time for the mixture reduction algorithms AKL (red), SKL (green) and ISE (blue) is given versus the number of remaining components $\textbf{M}$ in the reduced mixture. The original density in the simulations has 25 components.  }}
